PointBeV: A Sparse Approach to BeV Predictions

Bird's-eye View (BeV) representations have emerged as the de-facto shared space in driving applications, offering a unified space for sensor data fusion and supporting various downstream tasks. However, conventional models use grids with fixed resolution and range and face computational inefficiencies due to the uniform allocation of resources across all cells. To address this, we propose PointBeV, a novel sparse BeV segmentation model operating on sparse BeV cells instead of dense grids. This approach offers precise control over memory usage, enabling the use of long temporal contexts and accommodating memory-constrained platforms. PointBeV employs an efficient two-pass strategy for training, enabling focused computation on regions of interest. At inference time, it can be used with various memory/performance trade-offs and flexibly adjusts to new specific use cases. PointBeV achieves state-of-the-art results on the nuScenes dataset for vehicle, pedestrian, and lane segmentation, showcasing superior performance in static and temporal settings despite being trained solely with sparse signals. We will release our code along with two new efficient modules used in the architecture: Sparse Feature Pulling, designed for the effective extraction of features from images to BeV, and Submanifold Attention, which enables efficient temporal modeling. Our code is available at https://github.com/valeoai/PointBeV.

==> figs/eval_sampling.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/eval_sampling.pdf}
    \caption{\textbf{Sampling stragies for evaluation.}
    \todo{change with real examples: please provide eloi with individual images}
    }
    \label{fig:eval_sampling}
\end{figure}

==> figs/fine_ps.tex <==
\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{figs/fine_ps.png}
    \caption{Evolution of the segmentation map prediction using different patch size durint the fine pass. The first row represents the predictions, the second row represents the activated points used during predictions. From left to right, we have on the first row: ground truth, predictions with fine patch size equals 1, 3, 5, 7, 9, 11 and 13. The higher the patch size, the more points are activated in the local context of anchor points
    \eloi{Les cartes de segmentation fig 6 7 8 semblent etre avant thresholding (effet de flou).}
    }
    \label{fig:fine_ps}
\end{figure*}

==> figs/fine_thresh.tex <==
\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{figs/fine_thresh.png}
    \caption{Evolution of the segmentation map prediction using different threshold to activate anchor points before the fine pass. The first row represents the predictions, the second row represents the activated points used during predictions. From left to right, we have on the first row: ground truth, predictions with threshold equals 0.0, 0.1, 0.2, 0.3, 0.4, 0.5. The lower the threshold, the more points are considered as anchor points.}
    \label{fig:fine_thresh}
\end{figure*}

==> figs/reduction.tex <==
\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{figs/reduction.png}
    \caption{Evolution of the segmentation map prediction using different reduction factor for the coarse pass. The higher is the reduction factor, the sparser are the points with ... \loick{Parler de fine patch adaptatif.} \todo{supprimer image en bas à gauche}}
    \label{fig:reduction}
\end{figure*}

